Knowledge Workers' Perspectives on AI Training for Responsible AI Use

AI expansion has accelerated workplace adoption of new technologies. Yet, it is unclear whether and how knowledge workers are supported and trained to safely use AI. Inadequate training may lead to unrealized benefits if workers abandon tools, or perpetuate biases if workers misinterpret AI-based outcomes. In a workshop with 39 workers from 26 countries specializing in human resources, labor law, standards creation, and worker training, we explored questions and ideas they had about safely adopting AI. We held 17 follow-up interviews to further investigate what skills and training knowledge workers need to achieve safe and effective AI in practice. We synthesize nine training topics participants surfaced for knowledge workers related to challenges around understanding what AI is, misinterpreting outcomes, exacerbating biases, and worker rights. We reflect how these training topics might be addressed under different contexts, imagine HCI research prototypes as potential training tools, and consider ways to ensure training does not perpetuate harmful values.

==> use_cases.tex <==
\begin{enumerate}
    \item \textit{Language translation }[P6, P7, P9, P10, P12, P16, P17]: 
    \item \textit{Drafting text} (e.g., concept notes, policies, arguments, training proposals, job descriptions): quote
    \item \textit{Image generation} [P4, P9]: "If we are having an event on one topic, we would ask colleagues who are working on graphic design to come up with an image. And they often use, I think, AI for that image...'okay, I would like a picture showing diverse people from different backgrounds getting together for a particular topic.'" (P9)
    \item \textit{Brainstorming training material} [P9, P10, P11, P12]: "[I have] given [it] learning materials that that's actually used in in a training workshop. And then I asked AI to...come up with multiple, multiple choices test to assess the learning of this, of this material." (P10)
    \item \textit{Enhancing, editing, reviewing human-drafted texts} [P1, P4, P9]: "I would type up the closing, and then I would ask chatGPT to, like, enhance it." (P1)% add requirements to old documentation (p1) %    \item Grammar [P4]: "I use ChatGPT to see my grammar, especially in English, I use also when we are building a message that we want to see if it's well done grammatically in Spanish or in English." (P4)
    \item \textit{Transcription, creating meeting agendas or notes} [P1, P5, P12, P17]: 
    \item \textit{Researching information} [P1, P12, P13, P14, P17]: "Training need analysis:...what kind of specified jobs [do] they need in Japan side...Now Japan [has] 14 sectors...industry like Marine and business...so we try to organize this training analysis need [for] all the guidelines..." (P12) %, e.g., analyzing sector needs for training
\end{enumerate}
